Sub-Chain Beam for mmWave Devices: A Trade-off between Power Saving and Beam Correspondence

Beam correspondence, or downlink-uplink (DL-UL) beam reciprocity, refers to the assumption that the best beams in the DL are also the best beams in the UL. This is an important assumption that allows the existing beam management framework in 5G to rely heavily on DL beam sweeping and avoid UL beam sweeping: UL beams are inferred from the measurements of the DL reference signals. Beam correspondence holds when the radio configurations are symmetric in the DL and UL. However, as mmWave technology matures, the DL and the UL face different constraints often breaking the beam correspondence. For example, power constraints may require a UE to activate only a portion of its antenna array for UL transmission, while still activating the full array for DL reception. Meanwhile, if the UL beam with sub-array, named as sub-chain beam in this paper, has a similar radiation pattern as the DL beam, the beam correspondence can still hold. This paper proposes methods for sub-chain beam codebook design to achieve a trade-off between the power saving and beam correspondence.

==> acronyms.tex <==
\DeclareAcronym{3GPP}{
	short=3GPP,
	long=3rd generation partnership project
}
\DeclareAcronym{ADC}{
	short=ADC,
	long=analog-to-digital converter
}
\DeclareAcronym{AMP}{
	short=AMP,
	long=approximate message passing
}
\DeclareAcronym{ANN}{
	short=ANN,
	long=artificial neural network
}
\DeclareAcronym{AoA}{
	short=AoA,
	long=angle-of-arrival
}
\DeclareAcronym{AoD}{
	short=AoD,
	long=angle-of-departure
}
\DeclareAcronym{APS}{
	short=APS,
	long=azimuth power spectrum
}
\DeclareAcronym{AR}{
	short=AR,
	long=augmented reality
}
\DeclareAcronym{AV}{
	short=AV,
	long=autonomous vehicle
}
\DeclareAcronym{BM}{
	short=BM,
	long=beam management
}
\DeclareAcronym{BS}{
	short=BS,
	long=base station
}
\DeclareAcronym{BSM}{
	short=BSM,
	long=basic safety message
}
\DeclareAcronym{CDF}{
	short=CDF,
	long=cumulative distribution function
}
\DeclareAcronym{CP}{
	short=CP,
	long=cyclic-prefix
}
\DeclareAcronym{CSI-RS}{
	short=CSI-RS,
	long=channel state information reference signal
}
\DeclareAcronym{DFT}{
	short=DFT,
	long=discrete Fourier transform
}
\DeclareAcronym{DL}{
	short=DL,
	long=downlink
}
\DeclareAcronym{EKF}{
	short=EKF,
	long=extended Kalman filter
}
\DeclareAcronym{DSRC}{
	short=DSRC,
	long=dedicated short-range communication
}
\DeclareAcronym{FDD}{
	short=FDD,
	long=frequency division duplex
}
\DeclareAcronym{FMCW}{
	short=FMCW,
	long=frequency modulated continuous wave
}
\DeclareAcronym{FoV}{
	short=FoV,
	long=field-of-view
}
\DeclareAcronym{GNSS}{
	short=GNSS,
	long=global navigation satellite system
}
\DeclareAcronym{IA}{
	short=IA,
	long=initial access
}
\DeclareAcronym{IMU}{
	short=IMU,
	long=inertial measurement unit
}
\DeclareAcronym{lidar}{
	short=lidar,
	long=light detection and ranging
}
\DeclareAcronym{LOS}{
	short=LOS,
	long=line-of-sight
}
\DeclareAcronym{LPF}{
	short=LPF,
	long=low pass filter
}
\DeclareAcronym{LTE}{
	short=LTE,
	long=long term evolution
}
\DeclareAcronym{MIMO}{
	short=MIMO,
	long=multiple-input multiple-output
}
\DeclareAcronym{ML}{
	short=ML,
	long=machine learning
}
\DeclareAcronym{mmWave}{
	short=mmWave,
	long=millimeter wave
}
\DeclareAcronym{MRR}{
	short=MRR,
	long=medium range radar
}
\DeclareAcronym{NLOS}{
	short=NLOS,
	long=non-line-of-sight
}
\DeclareAcronym{NB}{
	short=NB,
	long=narrow beam
}
\DeclareAcronym{NR}{
	short=NR,
	long=new radio
}
\DeclareAcronym{OFDM}{
	short=OFDM,
	long=orthogonal frequency-division multiplexing
}
\DeclareAcronym{ppm}{
	short=ppm,
	long=parts-per-million
}
\DeclareAcronym{PF}{
	short=PF,
	long=particle filter
}
\DeclareAcronym{RMS}{
	short=RMS,
	long=root-mean-square
}
\DeclareAcronym{RPE}{
	short=RPE,
	long=relative precoding efficiency
}
\DeclareAcronym{RS}{
	short=RS,
	long=reference signal
}
\DeclareAcronym{RSRP}{
	short=RSRP,
	long=reference signal received power
}
\DeclareAcronym{RSU}{
	short=RSU,
	long=roadside unit
}
\DeclareAcronym{SCS}{
	short=SCS,
	long=subcarrier spacing
}
\DeclareAcronym{SNR}{
	short=SNR,
	long=signal-to-noise ratio
}
\DeclareAcronym{SRS}{
	short=SRS,
	long=sounding reference signal
}

\DeclareAcronym{SSB}{
	short=SSB,
	long=synchronization signal block
}
\DeclareAcronym{THz}{
	short=THz,
	long=terahertz
}
\DeclareAcronym{UAV}{
	short=UAV,
	long=unmanned aerial vehicle
}
\DeclareAcronym{UE}{
	short=UE,
	long=user equipment
}
\DeclareAcronym{UKF}{
	short=UKF,
	long=unscented Kalman filter
}
\DeclareAcronym{UL}{
	short=UL,
	long=uplink
}
\DeclareAcronym{ULA}{
	short=ULA,
	long=uniform linear array
}
\DeclareAcronym{V2I}{
	short=V2I,
	long=vehicle-to-infrastructure
}
\DeclareAcronym{V2V}{
	short=V2V,
	long=vehicle-to-vehicle
}
\DeclareAcronym{V2X}{
	short=V2X,
	long=vehicle-to-everything
}
\DeclareAcronym{VR}{
	short=VR,
	long=virtual reality
}
\DeclareAcronym{VRU}{
	short=VRU,
	long=vulnerable road user
}
\DeclareAcronym{WB}{
	short=WB,
	long=wide beam
}



